On Synchronization of Wireless Acoustic Sensor Networks in the Presence of Time-varying Sampling Rate Offsets and Speaker Changes

A wireless acoustic sensor network records audio signals with sampling time and sampling rate offsets between the audio streams, if the analog-digital converters (ADCs) of the network devices are not synchronized. Here, we introduce a new sampling rate offset model to simulate time-varying sampling frequencies caused, for example, by temperature changes of ADC crystal oscillators, and propose an estimation algorithm to handle this dynamic aspect in combination with changing acoustic source positions. Furthermore, we show how deep neural network based estimates of the distances between microphones and human speakers can be used to determine the sampling time offsets. This enables a synchronization of the audio streams to reflect the physical time differences of flight.

==> commands.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = Schmalen2020.tex
% !TeX program = pdflatex
% !BIB program = bibtex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\zB}{z.~B.\xspace}
\newcommand{\dhAbbrev}{d.~h.\xspace}
\newcommand{\vgl}{vgl.\xspace}
\newcommand{\sog}{sog.\xspace}
\newcommand{\ua}{u.~a.\xspace}
\newcommand{\bspw}{bspw.\xspace}
\newcommand{\bzw}{bzw.\xspace}
\newcommand{\ca}{ca.\xspace}
\newcommand{\ggf}{ggf.\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% basic math style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\grad}{\ensuremath{^\circ}}
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\scr}[1]{\ensuremath{\mathcal{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mathematical operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\sinc}{sinc}
\renewcommand{\Re}{Re}
\renewcommand{\Im}{Im}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\ee}{\mathrm e}
\newcommand{\jj}{\mathrm j}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rect}{\ensuremath{{\rm rect}}}
\newcommand{\sgn}{\ensuremath{{\rm sgn}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% fourier-transformation, z-transformation 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\FT}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\text{---}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IFT}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\text{---}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}
\newcommand{\ZT}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\overset{z}{\text{---}}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IZT}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\overset{z^{-1}}{\text{---}}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}
\newcommand{\ZTE}{\hspace{0.3cm}{\circ}\hspace{-.4mm}{\overset{z_1}{\text{---}}}{\hspace{-1mm}}{\bullet}\hspace{0.3cm}}
\newcommand{\IZTE}{\hspace{0.3cm}{\bullet}\hspace{-.4mm}{\overset{z_1^{-1}}{\text{---}}}{\hspace{-.4mm}}{\circ}\hspace{0.3cm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% other
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\SNR}{\ensuremath{{\rm SNR}}}
\newcommand{\SINR}{\ensuremath{{\rm SINR}}}
\newcommand{\Prob}{\ensuremath{{\rm Prob}}}
\newcommand{\rb}[1]{\raisebox{1.5ex}[-1.5ex]{#1}}
\newcommand{\erf}{\ensuremath{{\rm erf}}}
\newcommand{\erfc}{\ensuremath{{\rm erfc}}}



%\newacronym{PESQ}{PESQ}{Perceptual Evaluation of Speech Quality}
%\newacronym{ATF}{ATF}{Acoustic Transfer Function}
%\newacronym{STFT}{STFT}{Short Time Fourier Transform}
%\newacronym{FFT}{FFT}{Fast Fourier Transform}
%\newacronym{IFFT}{IFFT}{Inverse Fast Fourier Transform}
%\newacronym{MVDR}{MVDR}{Minimum Variance Distortionless Response}
%\newacronym{DSB}{DSB}{Delay-and-Sum Beamformer}
%\newacronym{TDOA}{TDOA}{Time Differences of Arrival}
%\newacronym{GEV}{GEV}{Generalized Eigenvalue}
%\newacronym{BAN}{BAN}{Blind Analytic Normalization}
%\newacronym{BLSTM}{BLSTM}{bi-directional Long Short-Term Memory}
%\newacronym{ReLU}{ReLU}{Rectified Linear Unit}
%\newacronym{FF}{FF}{feed-forward}
%\newacronym{SNR}{SNR}{signal-to-noise ratio}
%
%\newacronym{SINR}{SINR}{Signal-to-Interference-Noise Ratio}

%\newacronym{SDR}{SDR}{signal-to-distortion ratio}
%\newacronym{DNN}{DNN}{Deep Neural Network}
%\newacronym{ASR}{ASR}{Automatic Speech Recognition}
%\newacronym{DOA}{DoA}{Direction-of-Arrival}
%\newacronym{CDR}{CDR}{Coherence-to-Diffuse-Ratio}
%\newacronym{GMM}{GMM}{Gaussian Mixture Model}
%\newacronym{WER}{WER}{word error rate}
%\newacronym{PSD}{PSD}{Power Spectral Density}
%\newacronym{CNN}{CNN}{Convolutional Neural Network}
%\newacronym{EM}{EM}{Expectation-Maximization}
%\newacronym{tf}{tf}{time frequency}
%\newacronym{gcc}{GCC}{generalized cross correlation}
%\newacronym{CE}{CE}{Cross-Entropy}
%\newacronym{WRN}{WRN}{Wide Residual Network}
%\newacronym{SRO}{SRO}{Sampling Rate Offset}
%\newacronym{ACD}{ACD}{Average Coherence Drift}
%\newacronym{WACD}{WACD}{Weighted Average Coherence Drift}
%\newacronym{WASN}{WASN}{Wireless Acoustic Sensor Networks}
%\newacronym{ADC}{ADC}{Analog-to-Digital Converter}
%\newacronym{VAD}{VAD}{Voice Activity Detection}
%\newacronym{RMSE}{RMSE}{Root Mean Square Error}
%\newacronym{OSM}{OSM}{Overlap-Save method}
%\newacronym{GaBP}{GaBP}{Gaussian Belief Propagation}
%\newacronym{WLAN}{WLAN}{Wireless Local Area Network}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Source code listings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings}
\usepackage{textcomp}
% define MATLAB highlighting
\lstdefinelanguage{matlabNT}{ alsoletter={...}, %
                              morekeywords={ % keywords
                              break,case,catch,continue,elseif,else,end,for,
                              function,global,if,otherwise,persistent,return,
                              switch,try,while,...},
                              comment=[l]\%,% the comment sign comments
                              morecomment=[l]..., % if a command is split over multiple lines
                              morestring=[m]', %strings
}[keywords,comments,strings]

% define the wanted font for all highlightings here
\def\lstbasicfont{\fontfamily{pcr}\selectfont}
\lstset{  language=matlabNT,                            % use our version of highlighting
          keywordstyle=\color[rgb]{0,0,1},              % keywords
          commentstyle=\color[rgb]{0.133,0.545,0.133},  % comments
          stringstyle=\color[rgb]{0.627,0.126,0.941},   % strings
          captionpos=b,                                 % the caption position --> b:bottom
          basicstyle={\lstbasicfont
                      \footnotesize
                      \color[rgb]{0,0,0}},              % use defined font, smaller size and default textcolor black
          showstringspaces=false,                       % do not emphasize spaces in strings
          tabsize=2,                                    % number of spaces of a TAB
          mathescape=true,escapechar=§,                 % escape to latex with §...§
          upquote=true,                                 % upright quotes
          aboveskip={1.5\baselineskip},                 % a bit of space above
          columns=fixed,                                % nice spacing
          %backgroundcolor=\color[rgb]{0.95,0.95,0.95},  % the background color will be light gray
          numbersep=3mm,                                % spacing between numbers and text/code
          numbers=left,                                 % numbers are left
          numberstyle=\tiny,                            % numbers are tiny
          frame=trbl,                                   % single frame at top, right, bottom and left, capital letters
                                                        % produce double-lined frames
          frameround=tttt,                              % round corners
          framexleftmargin=6mm,                         % tweak margins
          xleftmargin=6mm,                              % tweak margins
          % the following is for replacing some matlab relations like >= or ~=
          % by the corresponding LaTeX symbols, which are much easier to read ...
          literate=%
            {~}{{$\neg$}}1            % \neg
            {<=}{{\tiny$\leq$}}1      % \leq
            {>=}{{\tiny$\geq$}}1      % \geq
            {~=}{{\tiny$\neq$}}1      % \neq
            {delta}{{\tiny$\Delta$}}1 % \Delta
}


==> sections/alternative_text.tex <==
\begin{table}[htb]
	\centering
	\setlength{\tabcolsep}{4pt}
	\begin{tabular}{l|c c c c|c c c c}
		\toprule	
		& \multirow{4}{*}{\rotatebox{90}{Diff. Pos.}}& \multirow{4}{*}{\rotatebox{90}{Silence}}& \multirow{4}{*}{\rotatebox{90}{$\Delta_\text{start} \neq 0$}}& \multirow{4}{*}{\rotatebox{90}{$\sigma_{OU}>0$}} &  &  & &\\
		& & & & &   & \multicolumn{3}{c}{RMSE}  \\
		& & & & &   & $\varepsilon $ & $\tau_\epsilon$ & $\tau_{\epsilon, \text{max}}$\\
		%\textbf{$\overline{\text{RMSE}}_\epsilon$} & \textbf{$\overline{\text{RMSE}}_{\tau_\epsilon}$} & \textbf{$\text{RMSE}_{\tau_\epsilon, \text{max}}$}\\	
		& & & & & \textbf{Method} & /\gls{ppm} & /samples& / samples\\	
		\midrule
		\multirow{4}{*}{\rotatebox{90}{Scenario-1}} &  & & &  & WACD &0.214 &0.135 &0.501 \\
		&  & & &  & DXCP-PhaT &0.15 &0.36 &0.68 \\
		&  & & &  & DXCP-PhaT$_8$ &0.69 &1.73 &3.65 \\
		&  & & &  & Proposed &0.40 &0.145 &0.495\\
		\midrule
		\multirow{4}{*}{\rotatebox{90}{Scenario-2}} &  & & & \cmark & WACD &0.565 &0.262 &0.697 \\
		&  & & & \cmark & DXCP-PhaT &0.56 &0.40 &1.04  \\
		&  & & & \cmark & DXCP-PhaT$_8$ &0.90 &1.71 &3.65 \\
		&  & & & \cmark & Proposed &0.50 &0.19 &0.69 \\
		\midrule
		\multirow{4}{*}{\rotatebox{90}{Scenario-3}} &  & & \cmark & \cmark & WACD &0.625 &0.732 &2.092 \\
		&  & & \cmark & \cmark & DXCP-PhaT &0.66 & 0.97 &2.73 \\
		&  & & \cmark & \cmark & DXCP-PhaT$_8$ &0.95 &1.83 &4.66 \\
		&  & & \cmark & \cmark & Proposed &0.51  & 0.273 &1.04\\
		\midrule
		\multirow{4}{*}{\rotatebox{90}{Scenario-4}} & \cmark &\cmark & \cmark & \cmark & WACD &2.980 &6.043 &20.999 \\
		& \cmark &\cmark & \cmark & \cmark & DXCP-PhaT &28.96 &21.84 &161.54 \\
		& \cmark &\cmark & \cmark & \cmark & DXCP-PhaT$_8$ &1.31 &2.70 &7.76 \\
		& \cmark &\cmark & \cmark & \cmark & Proposed &0.57 &0.32 &1.20 \\
		\midrule
		\multirow{4}{*}{\rotatebox{90}{Scenario-5}} & \cmark & & \cmark & \cmark & WACD &2.800 &3.248 &10.963\\
		& \cmark & & \cmark & \cmark & DXCP-PhaT &22.42 &16.61 &160.49 \\
		& \cmark & & \cmark & \cmark & DXCP-PhaT$_8$ &1.28 &2.81 &6.93\\
		& \cmark & & \cmark & \cmark & Proposed &0.64 &0.32 &1.10 \\
		\bottomrule
	\end{tabular}
\end{table} 


==> sections/dynamic_wacd.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = icassp22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Dynamic Weighted Average Coherence Drift}
%\begin{align}
%	\Phi_{gh}^\tau(\ell B_s, k) {=}
%	&\frac{1}{\nu_W} \!  \sum\limits_{\kappa=0}^{\nu_W-1} \! Y_g(\ell B_s{+}\kappa B_W, k) Y_h^*(\ell B_s{+}\kappa B_W{+}\tau, k). \\  &\text{with } g, h \in\{1, 2\} \nonumber
%\end{align}
%\begin{align}
%	W_{12}(\ell, k) {\approx} \frac{\sum\limits_{\kappa=0}^{\nu_W- 1}|X^{(m)}(\ell B_s, k)|^2\cdot \exp\left(j\frac{2 \pi k}{N} \kappa B_W \sro{12}{\ell} \right)}{\sqrt{\overline{|Y_1(\ell B_s {+}\kappa B_W, k)|^2} \cdot \overline{|Y_2(\ell B_s {+}\kappa B_W {+} \tau, k)|^2}}}.
%\end{align}
%with 
%\begin{align}
%	\overline{|Y_g(\ell B_s, k)|^2} = \sum\limits_{\kappa=0}^{\nu_W- 1}\!|Y_2(\ell B_s{+}\kappa B_W{+}\tau, k)|^2
%\end{align}
%\begin{align}
%	\Gamma^\tau_{12}(\ell B_s, k) &\approx  H_{12}^{(m)}(k) \cdot W_{12}(\ell, k) \cdot \exp{\left(j\frac{2 \pi k}{N}\tauwacd{12}{\ell}\right)}
%\end{align}
%\begin{align}
%	&Y_2(\ell B_s{+}\kappa B_W {+}\tau , k) \rightarrow \nonumber \\
%	&Y_2(\ell B_s{+}\kappa B_W {+}\tau , k) \cdot \exp{\left(-j \frac{2\pi k}{N}  \kappa B_W \estsro{12}{\ell-1} \right)}
%\end{align}

\begin{itemize}
	\item Adaptation of the online \gls{WACD} method we presented in~\cite{Chinaev2021} to dynamic problem with speech pauses, position changes and time-varying \gls{SRO}
	\item First step coarse synchronization (compensate whole-sample offset):
	\begin{itemize}
		\item Start sync when source activity is detected for one microphone signal for the first time 
		\item Offset to be compensated found by searching for maximum of cross-correlation similar to~\cite{miyabe13}
		\item Difference to~\cite{miyabe13}: Correlation not calculated for whole signal rather for the first \SI{20}{\second} with speech activity
		\item Note that the estimated offset results from $\tausto$ and an average position dependent delay
	\end{itemize}
	\item In the following the concept of the online \gls{WACD} for \gls{SRO} estimation presented in \cite{Chinaev2021} is recapitulated shortly
	\item Foundation: block-oriented coherence estimation(for sake of simplicity fixed position, block shift $B_s$, block index $\ell$)
	\begin{align}
		\Gamma^\tau_{12}(\ell B_s, k) &= \frac{\Phi^\tau_{12}(\ell B_s, k)}{\sqrt{\Phi^0_{11}(\ell B_s, k) \cdot \Phi^0_{22}(\ell B_s+\tau, k)}}
	\end{align}
	\begin{itemize}
		\item $\tau$ = adjustable parameter to coarsely compensate the \gls{SRO}-induced signal delay% $\taueps{n}$
%		\item Note that the discrete time index $n$ is used instead of a block index $\ell$ to define the temporal position of the considered block due to the adjustable shift of the analysis window $\tau$ 
	\end{itemize}
	\item \Glspl{PSD} estimated via a Welch method:
	\begin{align}
		\Phi_{gh}^\tau(\ell B_s, k) {=}
		&\frac{1}{\nu_W} \!  \sum\limits_{\kappa=0}^{\nu_W-1} \! Y_g(\ell B_s{+}\kappa B_W, k) Y_h^*(\ell B_s{+}\kappa B_W{+}\tau, k). \\  &\text{with } g, h \in\{1, 2\} \nonumber
	\end{align}
	with
%	\begin{align}
%		Y_g(n, k) = \sum_{\tilde{n}=n}^{n+N} y_g[\tilde{n}] \cdot \exp\left(-j\frac{2 \pi k}{N}\tilde{n}\right)
%	\end{align}
	\begin{align}
		\nu_W = \left\lfloor \frac{N_W-N+B_W}{B_W} \right\rfloor
	\end{align}
	\item Resulting coherence (see~\cite[Eq. (23)]{SchHaeb2017})
	\begin{align}
	\Gamma^\tau_{12}(\ell B_s, k) &\approx  H_{12}^{(m)}(k) \cdot W_{12}(\ell, k) \cdot \exp{\left(j\frac{2 \pi k}{N}\tauwacd{12}{\ell}\right)}
	\end{align}
	with
	\begin{align}
	H_{12}^{(m)}(k) = H_1^{(m)}(k)\cdot \left(H_2^{(m)}(k)\right)^*
	\end{align}
	\begin{align}
		W_{12}(\ell, k) {\approx} \frac{\sum\limits_{\kappa=0}^{\nu_W- 1}|X^{(m)}(\ell B_s, k)|^2\cdot \exp\left(j\frac{2 \pi k}{N} \kappa B_W \sro{12}{\ell} \right)}{\sqrt{\overline{|Y_1(\ell B_s, k)|^2} \cdot \overline{|Y_2(\ell B_s +\tau, k)|^2}}}.
	\end{align}
	with (divide by $\nu_W$)
	\begin{align}
		\overline{|Y_g(\ell B_s, k)|^2} = \sum\limits_{\kappa=0}^{\nu_W- 1}\!|Y_g(\ell B_s{+}\kappa B_W, k)|^2
	\end{align}
%	\begin{align}
%		|Y_i(n, k)|^2 = |H_i(k)|^2\cdot |X^{(m)}(n, k)|^2 + |V_i(n, k)|^2
%	\end{align}
%	\begin{align}
%		\tauwelch{\varepsilon}{\kappa} = \kappa B_W \varepsilon
%	\end{align}
	and average delay within block:
	\begin{align}
		\tauwacd{12}{\ell} = - \tausto - \tau +  \frac{N_W}{2} \avgsro{12}{0} + \underset{\tilde{\ell} > 0}{\sum_{\tilde{\ell}=1}^{\ell}} \avgsro{12}{\tilde{\ell}} \cdot B_s
	\end{align}
	\item Note that $H_{12}^{(m)}(k)$ induces $\taugeo^{(m)}$ 
	\item Complex conjugate product of consecutive coherence functions:
	\begin{align}
		\cp{\ell} = \Gamma^{\taucomp{12}{\ell}}_{12}(\ell B_s, k) \cdot \left(\Gamma^{\taucomp{12}{\ell}}_{12}((\ell-\tmpdist) B_s, k)\right)^*
	\end{align}
	(why differentiate between $\tauwacd{12}{\ell}$ and $\taucomp{12}{\ell}$?)
	\begin{itemize}
		\item $\taucomp{12}{\ell}$ is used for a coarse compensation of the \gls{SRO}-induced (whole-sample) delay based on \gls{SRO} estimates of previous blocks
		\begin{align}
			\taucomp{12}{\ell} = \left\lfloor\frac{N_W}{2} \cdot \estsro{12}{0}+  \underset{\tilde{\ell} > 0}{\sum_{\tilde{\ell}=1}^{\ell}} B_S \cdot \estsro{12}{\tilde{\ell}}\right\rceil
		\end{align}
	\end{itemize}
	\item See~\cite[Eq. (14)]{SchHaeb2017} (Slowly changing \gls{SRO} is approximated as constant during the interval $[(\ell - \tmpdist) B_s,  \ell B_s]$):
	\begin{align}
		\cp{\ell,k} \approx  W_\text{SNR}(\ell, k) \cdot \exp{\left(j \frac{2\pi k}{N}  \tmpdist B_s \avgsro{12}{\ell} \right)}
	\end{align}
%	\begin{align}
%		\cp{\ell,k} = W_\text{SNR}(\ell, k) \cdot \exp{\left(j \frac{2\pi k}{N} \sum_{\tilde{n}=n + \frac{N_W}{2} - N_d}^{n + \frac{N_W}{2}} \sro{12}{\tilde{n}}\right)}
%	\end{align}
%	\item Assuming that the \gls{SRO} is approximately constant within one block:
%	\begin{align}
%		\cp{\ell,k} \approx  W_\text{SNR}(\ell, k) \cdot \exp{\left(j \frac{2\pi k}{N} N_d \cdot \sro{12}{\ell} \right)}
%	\end{align}
	\item Temporally weighted averaged phase information similar to~\cite{SchHaeb2017}:
	\begin{align}
		\wacd{\ell,k} = \alpha \cdot \wacd{\ell-1,k} + (1-\alpha) \cdot \cp{\ell,k}
	\end{align}
	\begin{itemize}
		\item Comparison to (online) \gls{WACD}:  Temporal weighting to be able to adapt faster to large/fast \gls{SRO} changes
		\item All time-frequency bins are individually weighted by $W_\text{SNR}(\ell, k)$ representing it's \gls{SNR}: 
		\begin{align}
		W_\text{SNR}(\ell, k) = |H_{12}^{(m)}(k)|^2 \cdot W_{12}(\ell, k) \cdot W_{12}^*(\ell-\tmpdist, k)
		\end{align}
		\item Initialization: $\wacd{-1,k} =0 \ \forall \ k$ 
	\end{itemize}
	\item As discussed in~\cite{SchHaeb2017} it is assumed for coherence drift based \gls{SRO} estimation that $W_\text{SNR}(\ell, k)$ does not contribute to the phase of $\cp{\ell,k}$ $\rightarrow$ Problems
	\begin{itemize}
		\item Position of source has to be constant during the interval needed to calculate $\cp{\ell,k}$
		\begin{itemize}
				\item Reduce window  $N_W$ and $\tempdist$ compared to \cite{Chinaev2021} in order to be able to utilize also signal parts where the source position is only static for a short period
		\end{itemize}
		\item \gls{SRO} has to be zero or at least close to zero
		\begin{itemize}
			\item Previously solved by the multi-stage approach using resampling~\cite{SchHaeb2017}
			\item Here: Use \gls{SRO} estimate of previous block $\estsro{12}{\ell-1}$ to resample the currently considered block of $y_2[n]$
			\item $Y_2(\ell B_s{+}\kappa B_W {+}\tau , k)$ is replaced by
			\begin{align}
				Y_2(\ell B_s{+}\kappa B_W {+}\tau , k) \cdot \exp{\left(-j \frac{2\pi k}{N}  \kappa B_W \estsro{12}{\ell-1} \right)}
			\end{align}
		\end{itemize}
	\end{itemize}
	\item Disadvantage of previously used phase-based \gls{SRO} estimation (polar-normalization): Phase ambiguity
	\begin{itemize}
		\item Limitation to an expected maximum \gls{SRO}
		\item Outliers may cause to phase wrap-around effects
	\end{itemize}
	\item Proposed: Interpretation of $\wacd{\ell,k}$ as \gls{GCC}~\cite{knapp76} with \gls{SNR}-based frequency weights
	\begin{align}
		&\estsro{12}{\ell} = \frac{\lambda_\text{max}}{\tmpdist B_s} \\
		&\text{with } \lambda_\text{max} = \underset{\lambda}{\text{argmax}} \ |\wacdtime{\ell, \lambda}| \nonumber \\
		&\text{ and } \wacdtime{\ell, \lambda} = \text{IFFT}(\wacd{\ell,k}) \nonumber
	\end{align}	 
	\item Problem: Resolution of whole-sample lag $\lambda$ too low for accurate \gls{SRO} estimation
	\begin{itemize}
		\item Solution: Evaluation of $\wacdtime{\ell, \lambda}$ for sub-sample lags $\tilde{\lambda} \in \mathbb{R}$ with a sufficient resolution
		\begin{align}
			\wacdtime{\ell, \tilde{\lambda}} = \frac{1}{N} \sum_{k=0}^{N-1} \wacd{\ell, k } \cdot \exp{\left(j\frac{2 \pi k}{N} \tilde{\lambda}\right)}
		\end{align}
		 \item Efficient search for maximum by golden section search in the interval $[\lambda_\text{max}-0.5,\lambda_\text{max}+0.5]$ 
	\end{itemize}
	\item Further adjustments to handle the dynamic scenario
	\begin{itemize}
		\item Speech pauses are detected using an energy-based voice activity detector; $\wacd{\ell,k}$ is only updated if speech is active in all signal blocks needed to calculate $\Gamma^\tau_{12}(\ell B_s, k)$ and $\Gamma^\tau_{12}((\ell - \tmpdist)B_s, k)$  using  75 \% speech activity within each of the blocks as threshold
		\item Introduce a settling time: \gls{SRO} is only estimated for $\ell \geq 40$, i.e., first \gls{SRO} estimate is produced after \SI{ 5.12}{\second}); \gls{SRO} changes very slowly  $\Rightarrow$ take over $\estsro{12}{40}$ as estimate for all blocks aggregated during settling time  ($\estsro{12}{\ell} = \estsro{12}{40} \ \forall \ \ell \in [0, 39]$))
	\end{itemize}
	\item TODO: List all Parameters (Rather in experiment section?)	
\end{itemize}

==> sections/introduction_old.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = icassp22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Introduction}
\label{sec:intro}

% WASN, Purpose
A \gls{WASN} is a composite of heterogeneous hardware for signal recording and processing, e.g., smartphones, tablets or smart home devices \cite{Akyildiz2002, Bertrand2011}. Because handheld devices can change their position, leave or enter the network due to their nature, the setup is only fixed for a certain period of time. For signal processing algorithms that require coherent signal streams, this implies techniques for a continuous synchronization of audio streams. 

One important aspect of audio stream synchronization is the utilized audio source itself. A spatially fixed source is a common choice \cite{Markovich-Golan2012, Miyabe2013, Bahari2017, Chinaev21_DXCPPhaT, Chinaev21_packet_loss} as it eases the synchronization problem. However, in smart environments humans move around and change their positions, while interacting with devices. In a scenario where the exact locations of a human speaker are not known, estimating a \gls{SRO} from signals of a moving source becomes a challenging task: Splitting the \gls{SRO} inflicted sample delays from the position change caused delays seems to be impossible without extra knowledge. A reasonable simplification is to focus on time periods where the position remains fixed and to skip transient phases, as proposed in
\cite{Araki19}. Here, we consider a similar scenario, where persons are at different random positions, e.g., speaking to a smart device, but remain at a fixed position if they are talking. Modeling and estimating movement phases are neglected to simplify the problem.

From our perspective synchronization includes estimating the \gls{SRO} and the \gls{STO} \cite{Chinaev2021}. While the first is caused by the different oscillation frequencies of the crystal oscillators driving the \glspl{ADC} on the devices, the latter depends on the unknown times the devices start to record the signals.

The actual frequency of a crystal oscillator is determined not only by the crystal cutting technique and its shape, but is influenced by a variety of environmental factors, e.g., aging, temperature, humidity and supply voltage \cite{Walls92}. While constant or slowly changing factors, such as aging, can be handled by assuming a constant \gls{SRO}, environmental factors such as temperature and supply voltage have a non-negligible impact on the  oscillator frequency \cite{QSL2021, SchJebHaeb2014}, which should be handled by a dynamic model.

However, the amount of publications investigating the physical sampling frequencies of different devices is limited, since hardware access to \glspl{ADC}, as exploited in \cite{SchJebHaeb2014} for example, is usually not available. The author of \cite{DRIFT2021} used GPS hardware as a timing source for accurate \gls{SRO} measurements of handheld devices and showed that typical \gls{SRO} values range between \SI{+416.84}{ppm} and \SI{-554.19}{ppm} for devices from renowned hardware manufacturers.
Publications on the transient nature of \glspl{SRO} are even more rare, since many publications conduct experiments in a controlled area for reproducibility and employ professional  equipment with excellent hardware, such that \glspl{SRO} seems to be a constant quantity. 

Assuming a constant \gls{SRO} enables long observation periods of several minutes, including smoothing operations, to derive a highly precise estimate \cite{Bahari2017, Chinaev21_DXCPPhaT}. However, as reported by the 
authors of \cite{QSL2021} a device usually requires a couple of minutes to settle after switching it on. During this settling time, the \gls{SRO} changes by several ppm, following an exponential decay curve that is affected by the temperature change of the circuit's parts. 

If signal processing in \glspl{WASN} is assumed to be a dynamic task \cite{Afifi2018marvelo}, the device's temperature will change by several degrees between phases of low energy consumption (deep sleep states) and intense processing phases with maximum power consumption. Hence, regarding the \gls{SRO} as a time-varying quantity seems to be reasonable in processing scenarios with changing computational workloads or rapid temperature changes originating from the environment.

For a complete synchronization, i.e., a synchronization that achieves to align all audio streams in a way as if they where recorded by a single soundcard with distributed microphones, \gls{SRO} and \gls{STO} information is required. Since \gls{STO} information is closely coupled with the relative positions of the human speakers towards the \gls{WASN}, this task requires location information or at least distance estimation as we will show later on.

The contributions of the paper are as follows: We use a discrete realization of an Ornstein-Uhlenbeck process to model a time-varying \gls{SRO} and propose a method to apply it to a signal. Furthermore, we discuss the necessary modifications to the previously proposed  \gls{SRO} estimation technique \textit{\gls{WACD}} to deal with time-varying \glspl{SRO}. 
In addition, we show how to utilize DNN-based distance estimates to derive a \gls{STO} estimate that regards the physical setup of the \gls{WASN}.





==> sections/problem.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = icassp22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Problem Statement}
\label{sec:problem}
\begin{itemize}
	\item Two sensor nodes recording acoustic sources at $M$ stationary positions
	\begin{itemize}
		\item Only one source active at any given time (no overlap) $\rightarrow$ Adaptation to multi-source case possible~\cite{CD_WLS}
		\item Pauses during positions/source change possible
	\end{itemize}
	\item Scenario = vivid but polite conversation between multiple humans in a smart home scenario
	\item Resulting microphone signals (continuous-time):
	\begin{align}
		\micsig{i}{(t)} = \sum_{m=1}^{M} \rir{i}{m}{t} \ast \srcsig{m}{t} + \noise{i}{t} \text{, with } i \in \{1, 2\}
	\end{align}
	with $\rir{i}{m}{t}$ = \gls{RIR} from  the $m$-th source position to the $i$-the sensor node, $\noise{i}{t}$ = sensor noise, $\srcsig{m}{t}$ = source signal for source at the $m$-th position ($\srcsig{m}{t}=0$ if source is not active)
	(Assumption: White sensor noise  + $v_1(t)$, $v_2(t)$ and $\srcsig{m}{t}$ are mutually uncorrelated)
	\item  Sampling (Difference to typical model: No "perfect" clock as reference $\rightarrow$ both microphones show an \gls{SRO} and start up delay) $\rightarrow$ time-discrete microphone signal\footnote{Taylor series/binomial approximation: $\frac{1}{1+x}= (1+x)^{-1} \approx 1 - x $ if $x \ll 1$}:
	\begin{align}
		\freq{i}{n} = \left(1 + \sro{i}{n}\right) \cdot f_s
	\end{align}
	\begin{align}
		\micsig{i}{[n]} &= \micsig{i}{\left(\delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1}{f_s\cdot(1+\sro{i}{\tilde{n}})}\right)}\nonumber \\ 
		  &\approx  \micsig{i}{\left(\delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1-\sro{i}{\tilde{n}}}{f_s}\right)}\nonumber \\ 
		   &= \micsig{i}{\left(\frac{n}{f_s} + \delay{i} - \sum_{\tilde{n}=0}^{n} \frac{\sro{i}{\tilde{n}}}{f_s}\right)}
	\end{align}
%	\begin{align}
%		t_{i}(n) &= \delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1}{f_s\cdot(1+\sro{i}{\tilde{n}})} \nonumber \\
%		&\approx \delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1-\sro{i}{\tilde{n}}}{f_s}\nonumber \\
%		&= \delay{i} + \frac{n}{f_s} - \sum_{\tilde{n}=0}^{n} \frac{\sro{i}{\tilde{n}}}{f_s}
%	\end{align}
	with time-varying \gls{SRO} $\sro{i}{n} << 1$ of microphone $i$  and  $\tau_i$ = point in time at which microphone $i$ starts recording
	\item Sampling with perfect clock ($\varepsilon_i=0$ and $T_i=0$):
	\begin{align}
		y_i^{(\text{sync})}[n] = \micsig{i}{\left(\frac{n}{f_s}\right)}
	\end{align}
	\item Comparison of $y_i^{(\text{sync})}[n]$ and $\micsig{i}{[n]}$ $\rightarrow$ signal is delayed by $\totaldelay{i}{n}$ samples with
	\begin{align}
		\totaldelay{i}{n} = - \delay{i} \cdot f_s +  \sum_{\tilde{n}=0}^{n} \sro{i}{\tilde{n}} 
	\end{align}
	\item Block-oriented processing / go to \gls{STFT}-domain (only valid if $\totaldelay{i}{n} \ll N$, where $N$ is the STFT frame size):
	\begin{itemize}
		\item \gls{SRO} changes only very slowly and, thus, can be approximated as constant during one \gls{STFT}-frame: $\sro{i}{n} \rightarrow \avgsro{i}{l}$ with  $l$ = Frame index
		\item Relationship to signal sampled with perfect clock:
		\begin{align} \label{EQ:SRO_Phase_Mult}
			Y_i(l B, k) \approx Y^{(\text{sync})}_\text{i}(l B, k)  \cdot \exp{\left(-j\frac{2 \pi k}{N} \avgtotaldelay{i}{l}\right)}
		\end{align}
		with 
		\begin{align}
			Y_\text{i}(l B, k) =  \sum_{n=0}^{N-1} y_i[l B + n] \cdot w[n] \cdot \exp\left(-j\frac{2 \pi k}{N}n\right)
		\end{align}
%		\begin{align}
%			Y^{(\text{sync})}_\text{i}(l, k) = H_i^{(m)}(k) \cdot X^{(m)}(l, k) + V_i(l, k)
%		\end{align}
		and average delay within the block
		\begin{align} \label{EQ:SRO_ACC}
   			\avgtotaldelay{i}{l} =  - \delay{i}\cdot f_s + \frac{N}{2} \avgsro{i}{0} + \underset{\tilde{l} > 0}{\sum_{\tilde{l}=1}^{l}} \avgsro{i}{\tilde{l}} \cdot B
		\end{align}
		with $k$ = frequency bin index; $N$ = FFT-size and $B$ = block shift
	\end{itemize}
	\item In the following (without loss of generality): Microphone 1 as reference + for sake of simplicity only $m$-th position (utilizing $\sro{1}{n}\ll 1$)
	\begin{align}
		\freq{2}{n} \approx \left(1 + \sro{12}{n}\right) \cdot \freq{1}{n}
	\end{align}
	(use index $l$, not $n$) where $\sro{12}{l} = \sro{2}{l} -\sro{1}{l}$.
	\item Goal: Sync audio streams so that physical delays induced by the different time of flights are preserved, e.g., needed for TDOA-based localization
	\begin{itemize}
		\item To be estimated: $\sro{12}{l}$, $\tausto = (\delay{2} - \delay{1})\cdot f_s$
		\item Additional Problem: Distinguish between $\tausto$  and $\taugeo^{(m)} = \frac{\dist{2}{m} - \dist{1}{m}}{c}$ with $\dist{i}{m}$ = distance between position of microphone $i$ and $m$-th source position and $c$ speed of sound
	\end{itemize}
%		\begin{align}
%			Y_2(l, k) \approx Y_\text{1}(l, k)  \cdot \exp{\left(-j\frac{2 \pi k}{N}\left(\taueps{l} + \taugeo - \tausto\right)\right)}
%		\end{align}
%		with $k$ = frequency bin index; $N$ = FFT-size and $B$ = block shift
%		\item At center of frame :
%		\begin{align}
%			\taueps{l} = \frac{N}{2} \sro{12}{0} + \underset{\tilde{l} > 0}{\sum_{\tilde{l}=1}^{l}} \sro{12}{\tilde{l}} \cdot B
%		\end{align}
%		with $\sro{12}{l} = \sro{2}{l} -\sro{1}{l}$, $\tausto = (\delay{2} - \delay{1})\cdot f_s$ and  $\taugeo = \frac{d_{2,m} - d_{1,m}}{c}$ with $d_{i,m}(l)$ = distance between position of microphone $i$ and $m$-th source position and $c$ speed of sound
	
\end{itemize}

==> sections/problem_js.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = ./../icassp22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Problem Statement} \label{sec:problem}
Let's assume a minimal setup of two sensor nodes recording acoustic sources at $M$ stationary positions, whereby only one source is active at any given time and short speech pauses are possible. Overlapping speech is not regarded, but may be handled similar to the multi-source case as described in \cite{CD_WLS}. Hence, the scenario can be interpreted as a polite conversation between multiple humans in a meeting or a smart home environment. The continuous-time microphone signals are 
\begin{align}
	\micsig{i}{(t)} = \sum_{m=1}^{M} \rir{i}{m}{t} \ast \srcsig{m}{t} + \noise{i}{t} \text{, with } i \in \{1, 2\}
\end{align}
with sensor noise $\noise{i}{t}$, source signal $\srcsig{m}{t}$ for source at the $m$-th position ($\srcsig{m}{t}=0$ if source is not active) and  $\rir{i}{m}{t}$ as the \gls{RIR} corresponding to the $m$-th position. It is assumed that the sensor noise is white and uncorrelated between the sensors.

Since each node has a non-perfect oscillator both microphone signals have an unknown \gls{STO} and an unknown \gls{SRO}. The impinging audio signal is sampled at the $i$-th node with a sampling frequency of 
	\begin{align}
		\freq{i}{n} = \left(1 + \sro{i}{n}\right) \cdot f_s
	\end{align}
deriving the $i$-th time-discrete microphone signal via the binomial approximation\footnote{Taylor series/binomial approximation: $\frac{1}{1+x}= (1+x)^{-1} \approx 1 - x $ if $x \ll 1$} with	
	\begin{align}
		\micsig{i}{[n]} &= \micsig{i}{\left(\delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1}{f_s\cdot(1+\sro{i}{\tilde{n}})}\right)} \\
		& \stackrel{*}{\approx}  \micsig{i}{\left(\delay{i} + \sum_{\tilde{n}=0}^{n}\frac{1-\sro{i}{\tilde{n}}}{f_s}\right)}\nonumber  
		   = \micsig{i}{\left(\frac{n}{f_s} + \delay{i} - \sum_{\tilde{n}=0}^{n} \frac{\sro{i}{\tilde{n}}}{f_s}\right)}
	\end{align}
where $f_s$ is the nominal sampling frequency, $\tau_i$ is the time at which microphone $i$ starts recording and $\sro{i}{n}$  is the time-varying \gls{SRO} of microphone $i$. Compared to a synchronously sampled signal at nominal frequency ($\varepsilon_i=0$ and $T_i=0$) 
\begin{align}
	y_i^{(\text{sync})}[n] = \micsig{i}{\left(\frac{n}{f_s}\right)}
\end{align}
the accumulating delay 
\begin{align}
\totaldelay{i}{n} = - \delay{i} \cdot f_s +  \sum_{\tilde{n}=0}^{n} \sro{i}{\tilde{n}} 
\end{align}
becomes obvious.

In the \gls{STFT}-domain signals are frame wise processed, whereby the \gls{SRO} temporal change compared to the \gls{STFT} frame size is negligible. Hence, we regard the average \gls{SRO} $\avgsro{i}{l}$ of frame $l$ in the following and describe the relationship between the signals via
		\begin{align} \label{EQ:SRO_Phase_Mult}
			Y_i(l B, k) \approx Y^{(\text{sync})}_\text{i}(l B, k)  \cdot \exp{\left(-j\frac{2 \pi k}{N} \avgtotaldelay{i}{l}\right)}
		\end{align}
		with 
		\begin{align}
			Y_\text{i}(l B, k) =  \sum_{n=0}^{N-1} y_i[l B + n] \cdot w[n] \cdot \exp\left(-j\frac{2 \pi k}{N}n\right)
		\end{align}
%		\begin{align}
%			Y^{(\text{sync})}_\text{i}(l, k) = H_i^{(m)}(k) \cdot X^{(m)}(l, k) + V_i(l, k)
%		\end{align}
		and average delay within the block
		\begin{align} \label{EQ:SRO_ACC}
   			\avgtotaldelay{i}{l} =  - \delay{i}\cdot f_s + \frac{N}{2} \avgsro{i}{0} + \underset{\tilde{l} > 0}{\sum_{\tilde{l}=1}^{l}} \avgsro{i}{\tilde{l}} \cdot B
		\end{align}
		with $k$ = frequency bin index; $N$ = FFT-size and $B$ = block shift. (only valid if $\totaldelay{i}{n} \ll N$)
		
In the following, without loss of generality the first microphone is selected as reference and the $m$-th position is regarded:
	\begin{align}
		\freq{2}{n} \approx \left(1 + \sro{12}{n}\right) \cdot \freq{1}{n}
	\end{align}
The task at hand can now be described as follows: Synchronize the two audio streams such that the physical delays induced by the different time of flights are preserved. So the two measures $\sro{12}{l} = \sro{2}{l} -\sro{1}{l}$ and $\tausto = (\delay{2} - \delay{1})\cdot f_s$ have to be estimated. Additionally, it has to be distinguished  between $\tausto$  and $\taugeo^{(m)} = \frac{\dist{2}{m} - \dist{1}{m}}{c}$ with $\dist{i}{m}$ being the distance between position of microphone $i$ and $m$-th source position and $c$ speed of sound.
